Domain-oriented Language Pre-training with Adaptive Hybrid Masking and Optimal Transport Alignment

Motivated by the success of pre-trained language models such as BERT in a broad range of natural language processing (NLP) tasks, recent research efforts have been made for adapting these models for different application domains. Along this line, existing domain-oriented models have primarily followed the vanilla BERT architecture and have a straightforward use of the domain corpus. However, domain-oriented tasks usually require accurate understanding of domain phrases, and such fine-grained phrase-level knowledge is hard to be captured by existing pre-training scheme. Also, the word co-occurrences guided semantic learning of pre-training models can be largely augmented by entity-level association knowledge. But meanwhile, by doing so there is a risk of introducing noise due to the lack of groundtruth word-level alignment. To address the above issues, we provide a generalized domain-oriented approach, which leverages auxiliary domain knowledge to improve the existing pre-training framework from two aspects. First, to preserve phrase knowledge effectively, we build a domain phrase pool as auxiliary training tool, meanwhile we introduce Adaptive Hybrid Masked Model to incorporate such knowledge. It integrates two learning modes, word learning and phrase learning, and allows them to switch between each other. Second, we introduce Cross Entity Alignment to leverage entity association as weak supervision to augment the semantic learning of pre-trained models. To alleviate the potential noise in this process, we introduce an interpretable Optimal Transport based approach to guide alignment learning. Experiments on four domain-oriented tasks demonstrate the superiority of our framework.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> background.tex <==
\section{Background}

\subsection{BERT}

\subsection{E-commerce Tasks}

\subsubsection{Review-based Question Answering}


\subsubsection{Aspect Extraction}


\subsubsection{Aspect Sentiment Classification}








==> temp.tex <==
\begin{table*}[th]
\small
\center
\caption{Performance comparison of baselines and our model on E-commerce downstream tasks (\%).}
\label{result}
\begin{tabular}{l|cccc|ccc|ccc|cc}
% \small
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Models\textbackslash{}Tasks}}} & \multicolumn{4}{c}{\textbf{Review QA}} & \multicolumn{3}{c}{\textbf{Product Classification}} & \multicolumn{3}{c}{\textbf{Review AE}} & \multicolumn{2}{c}{\textbf{Review ASC}} \\  
\multicolumn{1}{c|}{} & \textit{P.}            & \textit{R.}           & \textit{F}\textsubscript{1}     &\textit{EM}      & \textit{Acc.}          & \textit{Micro-F}\textsubscript{1}           & \textit{Macro-F}\textsubscript{1}          & \textit{P.}           & \textit{R.}           & \textit{F}\textsubscript{1}           & \textit{Acc.}                    & \textit{Macro-F}\textsubscript{1}           \\ \midrule
% \multicolumn{1}{c|}{}                                                         & $P.$            & $R.$           & $F1$     &$EM$      & $Acc.$          & $MiF1$          & $MaF1$          & $P.$           & $R.$           & $F1$           & $Acc.$                    & $MaF1$           \\ \midrule
% \multicolumn{1}{c|}{}                                                         & P.            & R          & F1           & Acc.          & Micro-F1          & MaF1          & P.           & R.           & F1           & P.           & R.           & F1           \\ \midrule
% \multicolumn{13}{c}{Pre-trained on Wiki by Huggingface.}
\multicolumn{13}{c}{Pre-trained on Wikipedia + BookCorpus by Huggingface.}                                    
\\  \midrule
BERT                                                                    & 58.91 &   62.18     &    60.69     &  40.22        & 66.54       & 81.90       & 78.82      & 83.15        & 84.66        & 83.90   & 86.01             & 62.87                         \\ \midrule
% \multicolumn{13}{c}{Post-trained on E-commerce corpus by us.}\\
\multicolumn{13}{c}{Further post-trained on E-commerce corpus by us.}\\
\midrule                                                             
BERT-PT                                                                & 60.28 &  62.25   & 61.25   & 41.23    & 67.84       & 81.98       & 79.28       & 84.33        & 84.09        & 84.81   & 86.40        &  64.96                 \\
% BERT-PT$^+$                                                                & 60.59 &  62.25   & 61.25   & 41.23    & 69.12       & 82.38       & 80.66       & 84.33        & 84.09        & 84.81   & 86.40        &  64.96                 \\
BERT-NP                                                            & 61.39 & 64.57          & 62.94        & 43.35 & 70.28       & 81.72       & 81.34   & 85.23        & 85.71        & 86.11       &  85.79        &  63.21                \\
SpanBERT                                                             & 62.52 &  64.77   &    63.63         & 43.94       & 71.59       & 81.51       & 81.50         & 85.67        & 86.22        & 86.23           & 86.76        &  65.13                \\  \midrule
% \\  \midrule
DP                                                                      & 63.76         & 67.02         & 65.77         & 44.63         &  75.07   & 85.84 &  86.28       & 86.80        & 89.47        & 88.11         &  87.84        &  69.02        \\
 % \midrule
\sahm                                                              &  65.18 & 68.30  & 66.18          & \textbf{45.56}        & 76.61   & 86.35 &  {87.32}        & \textbf{87.42}        & \textbf{90.55}       & \textbf{88.96}    & \textbf{89.17}  &  \textbf{70.35}                 \\
\snpa                                                              &  65.18 & 68.30  & 66.18          & \textbf{45.56}        & 76.61   & 86.35 &  {87.32}        & \textbf{87.42}        & \textbf{90.55}       & \textbf{88.96}    & \textbf{89.17}  &  \textbf{70.35}                 \\
\snpo                                                              &  65.18 & 68.30  & 66.18          & \textbf{45.56}        & 76.61   & 86.35 &  {87.32}        & \textbf{87.42}        & \textbf{90.55}       & \textbf{88.96}    & \textbf{89.17}  &  \textbf{70.35}                 \\
\sahm+\snpo                                                         & \textbf{66.71} & \textbf{70.13}         & \textbf{68.77}        &  45.40 &   \textbf{78.74}   & \textbf{90.37} &  \tb{90.94}   & 87.35         & 89.61         & 88.42  & 88.43         & 69.32                 \\
% K-BERT (MedicalKG)                                                             & -             & -            & -            & -           & -           & -           & -            & -            & -            &  94.1        & 94.3           & \textbf{94.2} \\ 
\bottomrule
\end{tabular}
\end{table*}

